A Good Start Matters: Enhancing Continual Learning with Data-Driven Weight Initialization

To adapt to real-world data streams, continual learning (CL) systems must rapidly learn new concepts while preserving and utilizing prior knowledge. When it comes to adding new information to continually-trained deep neural networks (DNNs), classifier weights for newly encountered categories are typically initialized randomly, leading to high initial training loss (spikes) and instability. Consequently, achieving optimal convergence and accuracy requires prolonged training, increasing computational costs. Inspired by Neural Collapse (NC), we propose a weight initialization strategy to improve learning efficiency in CL. In DNNs trained with mean-squared-error, NC gives rise to a Least-Square (LS) classifier in the last layer, whose weights can be analytically derived from learned features. We leverage this LS formulation to initialize classifier weights in a data-driven manner, aligning them with the feature distribution rather than using random initialization. Our method mitigates initial loss spikes and accelerates adaptation to new tasks. We evaluate our approach in large-scale CL settings, demonstrating faster adaptation and improved CL performance.

==> figures/speed.tex <==
\begin{wrapfigure}[15]{t}{0.45\textwidth} %16
    \vspace{-1.5cm}
       \includegraphics[width=\linewidth]{images/speed_new_err.png}
       \vspace{-0.7cm}
       \caption{Data-driven initialization reaches 95\% of the best accuracy of random initialization using $7\times$ less iterations. To demonstrate efficiency gain, we train models on first CL task for 3K iterations.
       }
       \label{fig:speed}
    \vspace{-1.5cm}
\end{wrapfigure}

==> tables/cl_methods.tex <==
\begin{wraptable}{r}{0.55\textwidth}
\vspace{-10pt}
\centering
\caption{\textbf{Impact of Weight Initialization on CL Methods.} An ImageNet-1K pre-trained ConvNeXtV2-F is incrementally trained on 5 CIL tasks from Places365-Std (73 classes per task). Rehearsal is used for DER++ but omitted for EWC. For both methods, compute is bounded by 600 iterations. For DER++, buffer is constrained by 24K samples. Accuracy is in \%.}
\label{tab:cl_methods_short}
\small
\begin{tabular}{c|ccc|ccc}
\toprule
\textbf{Weight Init} &
\multicolumn{3}{c|}{\textbf{EWC}} &
\multicolumn{3}{c}{\textbf{DER++}} \\
& 
$\boldsymbol{\mathcal{L}}_{\text{new}}$ & 
$\boldsymbol{\mathcal{A}}_{\text{new}}$ &  
$\boldsymbol{\mathcal{A}}_{\text{all}}$ &  
$\boldsymbol{\mathcal{L}}_{\text{new}}$ & 
$\boldsymbol{\mathcal{A}}_{\text{new}}$ & 
$\boldsymbol{\mathcal{A}}_{\text{all}}$ \\
\midrule
Random & 2.06 & 47.46 & 42.18 & 2.15 & 50.25 & 63.21 \\
Class Mean & 1.36 & 59.38 & 41.38 & 1.36 & 58.22 & 63.84 \\
\textbf{Least Square} & \textbf{1.28} & \textbf{60.65} & \textbf{42.57} & \textbf{1.34} & \textbf{58.70} & \textbf{64.23} \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{wraptable}


==> tables/resnet.tex <==
\begin{wraptable}{r}{0.55\textwidth} %0.65
\vspace{-30pt}
\centering
\caption{\textbf{ResNet Results.} 
An ImageNet-1K pre-trained ResNet18 incrementally learns 5 disjoint tasks from Places365-Std (73 classes per task). %using CE loss and last-layer plastic setting. 
Accuracy is reported in \%. 
$\mathcal{U}$ and $\mathcal{S}$ denote compute and storage constraints, respectively.}
\label{tab:last_layer_resnet}
\small
\begin{tabular}{ccccccc}
\toprule
\textbf{Weight Init} & $\boldsymbol{\mathcal{U}}$ & $\boldsymbol{\mathcal{S}}$ & $\boldsymbol{\mathcal{L}}_{\text{new}} \downarrow$ & $\boldsymbol{\mathcal{A}}_{\text{new}} \uparrow$ & $\boldsymbol{\mathcal{A}}_{\text{old}} \uparrow$ & $\boldsymbol{\mathcal{A}}_{\text{all}} \uparrow$ \\
\midrule
Random &       &       & 4.82 & 10.79 & 54.55 & 49.95 \\
Class Mean & 1200 & 192K & 1.69 & 21.17 & 54.23 & 50.70 \\
\textbf{Least Sq.} &    &      & \textbf{1.34} & \textbf{24.41} & \textbf{57.39} & \textbf{53.94} \\
\midrule
Random &       &       & 6.18 & 3.60  & 52.90 & 47.68 \\
Class Mean & 600  & 24K  & 1.44 & 12.08 & 51.97 & 47.71 \\
\textbf{Least Sq.} &    &      & \textbf{1.15} & \textbf{16.46} & \textbf{56.34} & \textbf{52.18} \\
\bottomrule
\end{tabular}
\vspace{-10pt}
\end{wraptable}


==> tables/weight_drift_short.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\vspace{-10pt} %-20pt
\centering
\caption{\textbf{Weight initializations in the first CL task.} An ImageNet-1K pre-trained model is adapted to the first CL task (73 classes from Places365-Std). %$\mathcal{A}_{\text{pre}}$ and $\mathcal{A}^{*}_{\text{pre}}$ denote ImageNet-1K accuracy (\%) using learned weights $W$ and analytical weights $W_{LS}$, respectively. 
$\mathcal{D}_{LS}$ quantifies the deviation of $W_{LS}$ from $W$ (Eq.~\ref{eq:ls_deviation}). %$C$ denotes \# of classes. %in the evaluation set. 
Accuracy is in \%.}
\label{tab:loss_comp_short}
\small
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c|c}
\toprule
\textbf{Weight Init} & $\boldsymbol{\mathcal{A}}_{\text{pre}}$ & $\boldsymbol{\mathcal{A}}_{\text{new}}$ & $\boldsymbol{\mathcal{A}}_{\text{old}}$ & $\boldsymbol{\mathcal{A}}_{\text{all}}$ & $\boldsymbol{\mathcal{D}}_{LS}$ \\
%& $C=1K$ & $C=73$ & $C=1K$ & $C=1073$ & $C=1K$ \\
\midrule
%\multicolumn{6}{l}{\textcolor{blue}{\textbf{MSE Loss}}} \\
\textcolor{orange}{\textbf{MSE Loss}} \\
Random       &     & 0.00  & 77.72 & 67.82 &       \\
Class Mean   & 77.72 & 50.29 & 68.34 & 66.04 & 377.18 \\
\textbf{Least Square} &  & \textbf{51.70} & 71.57 & \textbf{69.04} &  \\
\midrule
%\multicolumn{6}{l}{\textcolor{blue}{\textbf{CE Loss}}} \\
\textcolor{orange}{\textbf{CE Loss}} \\
Random       &     & 0.00  & 78.23 & 68.26 &       \\
Class Mean   & 78.23 & 21.10 & 77.87 & 70.64 & \textbf{78.97} \\
\textbf{Least Square} &  & \textbf{48.37} & 75.83 & \textbf{72.33} &  \\
\bottomrule
\end{tabular}%
}
\vspace{-20pt} %-30pt
\end{wraptable}

